Requirements Quality Research: a harmonized Theory, Evaluation, and Roadmap

High-quality requirements minimize the risk of propagating defects to later stages of the software development life cycle. Achieving a sufficient level of quality is a major goal of requirements engineering. This requires a clear definition and understanding of requirements quality. Though recent publications make an effort at disentangling the complex concept of quality, the requirements quality research community lacks identity and clear structure which guides advances and puts new findings into an holistic perspective. In this research commentary we contribute (1) a harmonized requirements quality theory organizing its core concepts, (2) an evaluation of the current state of requirements quality research, and (3) a research roadmap to guide advancements in the field. We show that requirements quality research focuses on normative rules and mostly fails to connect requirements quality to its impact on subsequent software development activities, impeding the relevance of the research. Adherence to the proposed requirements quality theory and following the outlined roadmap will be a step towards amending this gap.

==> material/affiliations.tex <==
\author*[1]{\fnm{Julian} \sur{Frattini}}\email{julian.frattini@bth.se}
\author[2]{\fnm{Lloyd} \sur{Montgomery}}\email{lloyd.montgomery@uni-hamburg.de}
\author[3,4]{\fnm{Jannik} \sur{Fischbach}}\email{jannik.fischbach@qualicen.de}

\author[1,5]{\fnm{Daniel} \sur{Mendez}}\email{daniel.mendez@bth.se}
\author[1]{\fnm{Davide} \sur{Fucci}}\email{davide.fucci@bth.se}
\author[1]{\fnm{Michael} \sur{Unterkalmsteiner}}\email{michael.unterkalmsteiner@bth.se}


\affil*[1]{
    %\orgdiv{Department of Software Engineering}, 
    \orgname{Blekinge Institute of Technology}, 
    \orgaddress{
        \street{Valhallvägen 1}, 
        \city{Karlskrona}, 
        %\postcode{37140}, 
        %\state{Blekinge}, 
        \country{Sweden}
    }
}

\affil[2]{
    \orgname{University of Hamburg}, 
    \orgaddress{
        %\city{Hamburg}, 
        %\postcode{20146}, 
        \country{Germany}
    }
}

\affil[3]{
    \orgname{Netlight Consulting GmbH}, 
    \orgaddress{
        \street{Sternstr. 5}, 
        \city{Munich}, 
        %\postcode{80538}, 
        %\state{Bavaria}, 
        \country{Germany}
    }}

\affil[4]{
    \orgname{University of Cologne}, 
    \orgaddress{
        \street{Albertus-Magnus-Platz}, 
        %\city{Cologne}, 
        %\postcode{50923}, 
        %\state{North-Rhine Westphalia}, 
        \country{Germany}
    }
}

\affil[5]{
    \orgname{fortiss GmbH}, 
    \orgaddress{
        \street{Guerickestraße 25}, 
        \city{Munich}, 
        %\postcode{80805}, 
        %\state{Bavaria}, 
        \country{Germany}
    }
}

==> material/tables/rqt-results.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|lr|lr|lr}
        Concept - Group & Code 1 & \# & Code 2 & \# & Code 3 & \# \\ \toprule
        Entity  & explicit & 33 & implicit & 24 & & \\ \hline
        Factor & & & & & & \\
        - Explicitness & explicit & 52 & implicit & 3 & referenced & 2 \\
        - Form & descriptive & 53 & formula & 4 & & \\
    \end{tabular}
    \caption{Distribution of codes among artifact-centric concepts}
    \label{tab:results:artifacts}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{l|p{1cm}r|lr|p{1cm}r|lr}
        Concept - Group & Code 1 & \# & Code 2 & \# & Code 3 & \# & Code 4 & \# \\ \toprule
        Stakeholder & N/A & 43 & reported & 12 & hypoth-esized & 2 & & \\ \hline
        Activity & ad hoc & 36 & systematic & 1 & N/A & 18 & unclear & 2 \\ \hline
        Attribute  & N/A & 49 & explicit & 7 & implicit & 1 & & \\ \hline
        Impact & & & & & & & & \\
        - Evidence & hypoth-esized & 19 & N/A & 17 & inductive & 11 & reference & 10 \\
        - Modality & deontic & 22 & epistemic & 18 & N/A & 17 & & \\
        - Comparative & absolute & 29 & N/A & 17 & compara-tive & 10 & mixed & 1 \\
        - Generalized & specific & 38 & N/A & 17 & mixed & 1 & general & 1 \\
    \end{tabular}
    \caption{Distribution of codes among activity-centric concepts}
    \label{tab:results:activities}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{l|lr|lr|lr|lr}
        Concept & Code 1 & \# & Code 2 & \# & Code 3 & \# & Code 4 & \# \\ \toprule
        Product & N/A & 43 & reported & 13 & hypothesized & 1 & & \\
        Process & N/A & 50 & reported & 6 & hypothesized & 1 & & \\
        Tools & N/A & 57 & & & & & & \\
        People & N/A & 47 & reported & 8 & hypothesized & 1 & reference & 1 \\
        Organization & N/A & 50 & reported & 7 & & & & \\
        Market & N/A & 49 & reported & 8 & & & & \\
    \end{tabular}
    \caption{Distribution of codes among context factors}
    \label{tab:results:context}
\end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{l|lr|lr|lr}
        Concept & Code 1 & \# & Code 2 & \# & Code 3 & \# \\ \toprule
        Cost & N/A & 48 & hypothesized & 6 & reference & 3 \\
        Resource & N/A & 52 & literal & 5 & & \\
    \end{tabular}
    \caption{Distribution of codes among economic concepts}
    \label{tab:results:economic}
\end{table}
